WarpSpeed: A High-Performance Library for Concurrent GPU Hash Tables

GPU hash tables are increasingly used to accelerate data processing, but their limited functionality restricts adoption in large-scale data processing applications. Current limitations include incomplete concurrency support and missing compound operations such as upserts. This paper presents WarpSpeed, a library of high-performance concurrent GPU hash tables with a unified benchmarking framework for performance analysis. WarpSpeed implements eight state-of-the-art Nvidia GPU hash table designs and provides a rich API designed for modern GPU applications. Our evaluation uses diverse benchmarks to assess both correctness and scalability, and we demonstrate real-world impact by integrating these hash tables into three downstream applications. We propose several optimization techniques to reduce concurrency overhead, including fingerprint-based metadata to minimize cache line probes and specialized Nvidia GPU instructions for lock-free queries. Our findings provide new insights into concurrent GPU hash table design and offer practical guidance for developing efficient, scalable data structures on modern GPUs.

==> applications.tex <==
\section{GPU applications}
\prashant{This section should be a single paragraph.}

%We now describe a few applications that can benefit from fully concurrent GPU hash tables. We also discuss a concrete API for concurrent hash tables needed by these applications.

% \hunterinline{cite CHORD/Napster here and google paper. And some CPU ops too.}
% Hash tables appear in virtually every domain and are used extensively on CPUs in domains such as databases~\cite{splinterDB,rocksdb2017partition, chordHashTable, consistentHashing}, graphs, and genomics.

% Many of these applications are designed to be run concurrently as this better maps to the CPU parallelism model. In some cases, such as \textit{k}-mer counting, the algorithm can't be run in a BSP format. 

% \hpdcaddition{There are many applications being ported to GPUs that can benefit from concurrent GPU hash tables. Databases~\cite{crystalGPUDatabase, gpuDatabaseSurvey, tqpGPUDatabase, KVGC} rely on hash tables for both data storage and efficient join processing~\cite{pumpUpTheVolume}. Sparse tensor contractions, commonly used in quantum and chemistry simulations, employ hash tables as an efficient solving method~\cite{hashedCoordinateTensors, AthenaSparseTensors, SpartaSparseTensors}. In genomics, hash tables play a crucial role in \textit{k}-mer counting and the \textit{k}-mer analysis phase of de-novo assembly~\cite{hofmeyr2020terabase, hashKmer, gpuKmerCounting, lockfreeKmerCount}. To efficiently process these datasets, concurrent upserts are essential.}



% \subsection{Data processing applications on GPUs}



% \begin{itemize}[leftmargin=*]
%     \item \textbf{Databases:} To minimize latency,
%       databases~\cite{gpuDatabaseSurvey, crystalGPUDatabase, tqpGPUDatabase}
%       run multiple transactions at once. Running transactions in a BSP format
%       serializes their launches, increasing latency and lowering throughput.
%       Databases like Crystal~\cite{crystalGPUDatabase} use tile-based
%       processing to process updates with atomic granularity. One critical use
%       of concurrent hash tables on the GPU is for processing database joins, as
%       was done in Lutz et al.~\cite{pumpUpTheVolume}.

%     \item \textbf{Databases:} Hash joins are a critical operation in OLAP
%       workloads, particularly when looking at unsorted data. Recent
%       papers~\cite{crystalGPUDatabase, gpuDatabaseSurvey, tqpGPUDatabase, KVGC}
%       run database operations on the GPU, including using hash tables to store
%       database information~\cite{KVGC}, and hash table join performance is
%       considered in Lutz et al.~\cite{pumpUpTheVolume}. These databases run
%       operations in a BSP format, which serializes launches, increasing latency
%       and lowering throughput. There is not yet a fully integrated hash join
%       inside of GPU databases, and concurrent GPU hash tables can fulfill this
%       need.

%     \item \textbf{Tensor contraction:} The data layout in tensor contraction
%       algorithms, like Correlated Coupled-Cluster Singles and Doubles
%       (CCSD)~\cite{tensorCCSD}, requires concurrent GPU hash table operations
%       in order to maintain performance and scalability. 
%       % Running these algorithms on GPUs~\cite{sparseTensorGPU} requires a
%       % departure from Bulk-synchronous operations. 
%       Additionally, the GPU hash table can be used to represent the output
%       sparse tensors~\cite{hashedCoordinateTensors, AthenaSparseTensors,
%       SpartaSparseTensors}. Tools like Sparta~\cite{SpartaSparseTensors} use a
%       hash table to accumulate output data during tensor contraction. This
%       accumulation step performs upsert operations that cannot be efficiently
%       translated to the BSP model.
    
%     \item \textbf{Genomics:} Hash tables are used in de-novo
%       assembly~\cite{hofmeyr2020terabase} and in \textit{k}-mer
%       counting~\cite{hashKmer, gpuKmerCounting, lockfreeKmerCount} for
%       representing large-scale genomics data. Both use cases require upserts to
%       be processed in incremental batches as the amount of data in flight is
%       larger than available memory.

% \end{itemize}

%\hunterinline{Papers to consider for citation: https://link.springer.com/article/10.1007/s10619-019-07280-z. Also there is a previous work about memory movement that considers hashing: https://dl.acm.org/doi/10.1145/3318464.3389705}

\subsection{Hash table API}

\begin{itemize}[leftmargin=*]
    % \item \textbf{\texttt{bool Insert(Key key, Val value):}} Insert adds a
  % copy of a key-value pair into the table. This typically does not check for
  % duplicate copies 
    % \noindent
    \item \textbf{\texttt{bool Upsert(key, value,func *callback):}}
      Upsert~\cite{libcuckoo, iceberg, clht} atomically adds a key-value pair to the table. If the key already exists, the callback function is executed to merge the old and new values.
      % is the generic implementation of
      % both "update" and "insert" and takes three parameters: a key to insert or
      % update, a value associated with the key, and a callback function that
      % determines what the upsert behavior should be. If the key does not exist,
      % it is inserted with the value. If it does exist, the callback function is
      % executed to determine the new value. 
      
      %Upsert can implement many different
     % operations based on the callback function, including insertions and
      % deletions. For example, the function \texttt{f()\{return;\}} is
      % equivalent to "insert if unique" and will not update the value if the key
      % already exists. The function \texttt{f(loc, key,
      % val)\{atomicAdd(\&loc->val, val);\}} will atomically accumulate every
      % value that matches the key, and the function \texttt{f(loc)\{loc.key =
      % tombstone;\}} implements deletion.

    % \noindent
    \item \textbf{\texttt{bool Query(key, value):}} Query locates an item in
      the hash table, returning true if it is found. If the key is found, the
      value associated with the key is returned.
    
\end{itemize}


==> ccs_and_keywords.tex <==
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>00000000.0000000.0000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>00000000.00000000.00000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>00000000.00000000.00000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>00000000.00000000.00000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc[300]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc[100]{Do Not Use This Code~Generate the Correct Terms for Your Paper}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Do, Not, Us, This, Code, Put, the, Correct, Terms, for,
  Your, Paper}

==> concurrency.tex <==
\section{Making hash tables concurrent}


*****DRAFTING *****

Converting a table from phased to concurrent requires






When a hash table has an associativity greater than one, locking is necessary to prevent duplicates of keys from existing in the table. To show this, consider two threads inserting a key K into a table with associativity 2. Let the possible locations K can map to be labeled A and B, with the insertion of A probing in the order A,B. 

\begin{lemma}

==> figures/bght_comp/bght_figure.tex <==
\begin{figure}[t]
    \centering
    \input{figures/bght_comp/bght_query}
    %\input{figures/bght_comp/bght_probe}

    \caption{Query performance for the phased implementation of the concurrent tables vs BGHT tables when run on 128-bit key-val pairs.}
    \label{fig::bght_all}
\end{figure}

==> figures/bght_comp/bght_probe.tex <==
\begin{subfigure}{.4\textwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    BGHTProbePlot,
    %ymode = log,
    %symbolic x coords={Insertion,Upsert,Query, Delletion},
    table/col sep = comma,
    enlarge x limits=0.15,
    xlabel={Load factor}
    ]

    %\addplot[p2ExtStyle, x=lf, y=query]   table {data/results/lf/p2_hashing_external.txt};

    %\addplot[p2ExtStyle, x index=0, y index=2] table {data/results/lf/p2_hashing_external.txt};
    \addplot[p2ExtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/p2_hashing_external.txt};

    % \addplot[p2IntStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/p2_hashing_internal.txt};
    
    \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/cuckoo_hashing.txt};


    \addplot[doubleStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/double_hashing.txt};

    \addplot[ihtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/iht_p2_hashing.txt};

    \addplot[ihtMetaStyle]  table[x expr=\thisrowno{0}, y expr=\thisrowno{2}]{data/results/lf_probe_bght/iht_p2_metadata_full_hashing.txt};

    \addplot[chainingStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/chaining_table.txt};

    %\addplot[warpcoreStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

    \addplot[p2MetaStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/p2_hashing_metadata.txt};


    \addplot[bchtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/bcht_8.txt};

    \addplot[p2bhtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/p2bht_8.txt};

    % \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe_bght/cuckoo_hashing.txt};




  \end{axis}
  \end{tikzpicture}
  \caption{BGHT Probe}
  \label{fig:bght_probe}
\end{subfigure}

==> figures/bght_comp/bght_query.tex <==
\begin{subfigure}{.4\textwidth}
\hspace*{-.4cm}
\begin{tikzpicture}
  \centering
  \begin{axis}[
    BGHTPlot,
    %ymode = log,
    %symbolic x coords={Insertion,Upsert,Query, Deletion},
    table/col sep = comma,
    enlarge x limits=0.15,
    xlabel={Load factor},
    ]

    %\addplot[p2ExtStyle, x=lf, y=query]   table {data/results/lf_bght/p2_hashing_external.txt};

    %\addplot[p2ExtStyle, x index=0, y index=2] table {data/results/lf_bght/p2_hashing_external.txt};
    \addplot[p2ExtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/p2_hashing_external.txt};

    % \addplot[p2IntStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/p2_hashing_internal.txt};

    \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/cuckoo_hashing.txt};


    \addplot[doubleStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/double_hashing.txt};

    \addplot[ihtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/iht_p2_hashing.txt};

    \addplot[ihtMetaStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/iht_p2_metadata_full_hashing.txt};

    \addplot[chainingStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/chaining_table.txt};

    %\addplot[warpcoreStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

    \addplot[p2MetaStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/p2_hashing_metadata.txt};

    \addplot[bchtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/bcht_8.txt};

    \addplot[p2bhtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/p2bht_8.txt};
    % \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_bght/cuckoo_hashing.txt};
  \end{axis}
  \end{tikzpicture}
  \caption{BGHT Query}
  \label{fig:bght_query}
\end{subfigure}

==> figures/churn/sawtooth_1.tex <==
\begin{subfigure}{2*\columnwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    graphPlot1,
    %ymode = log,
symbolic x coords={Upsert,Query, Deletion},
    enlarge x limits=0.15,
    legend to name=sawtoothLegend,
    legend columns = 2,
    xlabel={Average Performance across 1 Iteration}
    ]

    %BETA OuroborosPVA OuroborosCS
    \addplot[draw=none, p2ExtStyleFill, x=op, y=perf]   table {data/results/sawtooth_1/p2_hashing_external.txt};

    \addplot[draw=none, p2IntStyleFill, x=op, y=perf]   table {data/results/sawtooth_1/p2_hashing_internal.txt};


    \addplot[draw=none, doubleStyleFill, x=op, y=perf]   table {data/results/sawtooth_1/double_hashing.txt};

    \addplot[draw=none, ihtStyleFill, x=op, y=perf]   table {data/results/sawtooth_1/iht_p2_hashing.txt};

    \addplot[draw=none, chainingStyleFill, x=op, y=perf]   table {data/results/sawtooth_1/chaining_table.txt};

    \addplot[draw=none, warpcoreStyleFill, x=op, y=perf]   table {data/results/sawtooth_1/warpcore_hashing.txt};

    \addplot[draw=none, p2MetaStyleFill, x=op, y=perf]   table {data/results/sawtooth_1/p2_metadata_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

    \legend{P2 Hashing (External), P2 Hashing (Internal), Double Hashing, Iceberg Hashing, Chaining, Warpcore, P2 Metadata}
  \end{axis}
  \end{tikzpicture}
  \caption{Performance for expansions only}
  \label{fig:sawtooth_1}
\end{subfigure}

==> figures/churn/sawtooth_10.tex <==
\begin{subfigure}{\columnwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    graphPlot1,
    %ymode=log,
symbolic x coords={Upsert,Query, Deletion},
    enlarge x limits=0.15,
    xlabel={Average Performance across 10 Iterations}
    ]

    %BETA OuroborosPVA OuroborosCS
    \addplot[draw=none, p2ExtStyleFill, x=op, y=perf]   table {data/results/sawtooth_10/p2_hashing_external.txt};

    \addplot[draw=none, p2IntStyleFill, x=op, y=perf]   table {data/results/sawtooth_10/p2_hashing_internal.txt};


    \addplot[draw=none, doubleStyleFill, x=op, y=perf]   table {data/results/sawtooth_10/double_hashing.txt};

    \addplot[draw=none, ihtStyleFill, x=op, y=perf]   table {data/results/sawtooth_10/iht_p2_hashing.txt};

    \addplot[draw=none, chainingStyleFill, x=op, y=perf]   table {data/results/sawtooth_10/chaining_table.txt};

    \addplot[draw=none, warpcoreStyleFill, x=op, y=perf]   table {data/results/sawtooth_10/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};
  \end{axis}
  \end{tikzpicture}
  \caption{Performance for expansions only}
  \label{fig:sawtooth_10}
\end{subfigure}

==> figures/churn/sawtooth_100.tex <==
\begin{subfigure}{\columnwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    graphPlot1,
    %ymode = log,
symbolic x coords={Upsert,Query, Deletion},
    enlarge x limits=0.15,
    xlabel={Average Performance across 100 Iterations}
    ]

    %BETA OuroborosPVA OuroborosCS
    \addplot[draw=none, p2ExtStyleFill, x=op, y=perf]   table {data/results/sawtooth_100/p2_hashing_external.txt};

    \addplot[draw=none, p2IntStyleFill, x=op, y=perf]   table {data/results/sawtooth_100/p2_hashing_internal.txt};


    \addplot[draw=none, doubleStyleFill, x=op, y=perf]   table {data/results/sawtooth_100/double_hashing.txt};

    \addplot[draw=none, ihtStyleFill, x=op, y=perf]   table {data/results/sawtooth_100/iht_p2_hashing.txt};

    \addplot[draw=none, chainingStyleFill, x=op, y=perf]   table {data/results/sawtooth_100/chaining_table.txt};

    \addplot[draw=none, warpcoreStyleFill, x=op, y=perf]   table {data/results/sawtooth_100/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};
  \end{axis}
  \end{tikzpicture}
  \caption{Performance for expansions only}
  \label{fig:sawtooth_100}
\end{subfigure}

==> figures/churn/sawtooth_1000.tex <==
\begin{subfigure}{\columnwidth}

    
\begin{tikzpicture}
  \centering
  \begin{axis}[
    graphPlot1,
    %ymode = log,
    xticklabels={Upsert, Positive Query, Negative Query, Deletion},
%symbolic x coords={Upsert, Positive Query, Negative, Deletion},
    %xticklabels from table{\datatable}{0},
    % x tick label style={rotate=-15,anchor=north, yshift=-.5em},
    x tick label style={anchor=north, yshift=-.2em},
    enlarge x limits=0.15,
    legend to name=sawtoothLegend,
    legend columns = 2,
    xlabel={Operation},
    ]


    \addplot[draw=none, doubleStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/double_hashing.txt};
    
    \addplot[draw=none, doubleMetaStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/double_hashing_metadata.txt};

    \addplot[draw=none, ihtStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/iht_p2_hashing.txt};
    \addplot[draw=none, ihtMetaStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/iht_p2_metadata_full_hashing.txt};

    \addplot[draw=none, p2ExtStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/p2_hashing_external.txt};
    \addplot[draw=none, p2MetaStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/p2_hashing_metadata.txt};

    \addplot[draw=none, cuckooStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/cuckoo_hashing.txt};
    
    \addplot[draw=none, chainingStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/chaining_table.txt};



    % \addplot[draw=none, warpcoreStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};
    % \addplot[draw=none, p2IntStyleFill, x=op, y=perf]   table {data/results/sawtooth_1000/p2_hashing_internal.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};
    \legend{\double, \doubleMeta, \iceberg, \icebergMeta, \power, \meta, \cuckoo, \chaining}
    
  \end{axis}
  \end{tikzpicture}
  \caption{Performance of various hash tables operations during aging.}
  \label{fig:sawtooth_1000}
\end{subfigure}

==> figures/churn_probe/probe_1.tex <==
\begin{subfigure}{\columnwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    ProbePlot1,
    ymode = log,
symbolic x coords={Upsert,Query,Delete},
    enlarge x limits=0.15,
    legend to name=probeLegend,
    legend columns = 2,
    xlabel={Average Probes across 1 Iteration}
    ]

    %BETA OuroborosPVA OuroborosCS
    \addplot[draw=none, p2ExtStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_1/p2_hashing_external.txt};

    \addplot[draw=none, p2IntStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_1/p2_hashing_internal.txt};

    \addplot[draw=none, doubleStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_1/double_hashing.txt};

    \addplot[draw=none, ihtStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_1/iht_p2_hashing.txt};

    \addplot[draw=none, chainingStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_1/chaining_table.txt};

    \addplot[draw=none, warpcoreStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_1/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

    \legend{P2 Hashing (External), P2 Hashing (Internal), Double Hashing, Iceberg Hashing, Chaining, Warpcore}
  \end{axis}
  \end{tikzpicture}
  \caption{Performance for expansions only}
  \label{fig:probe_1}
\end{subfigure}

==> figures/churn_probe/probe_10.tex <==
\begin{subfigure}{\columnwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    ProbePlot1,
    ymode = log,
symbolic x coords={Upsert,Query,Delete},
    enlarge x limits=0.15,
    xlabel={Average Probes across 10 Iterations}
    ]

    %BETA OuroborosPVA OuroborosCS
    \addplot[draw=none, p2ExtStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_10/p2_hashing_external.txt};

    \addplot[draw=none, p2IntStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_10/p2_hashing_internal.txt};

    \addplot[draw=none, doubleStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_10/double_hashing.txt};

    \addplot[draw=none, ihtStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_10/iht_p2_hashing.txt};

    \addplot[draw=none, chainingStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_10/chaining_table.txt};

    \addplot[draw=none, warpcoreStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_10/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

  \end{axis}
  \end{tikzpicture}
  \caption{Performance for expansions only}
  \label{fig:probe_10}
\end{subfigure}

==> figures/churn_probe/probe_100.tex <==
\begin{subfigure}{\columnwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    ProbePlot1,
    ymode = log,
symbolic x coords={Upsert,Query,Delete},
    enlarge x limits=0.15,
    xlabel={Average Probes across 100 Iterations}
    ]

    %BETA OuroborosPVA OuroborosCS
    \addplot[draw=none, p2ExtStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_100/p2_hashing_external.txt};

    \addplot[draw=none, p2IntStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_100/p2_hashing_internal.txt};

    \addplot[draw=none, doubleStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_100/double_hashing.txt};

    \addplot[draw=none, ihtStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_100/iht_p2_hashing.txt};

    \addplot[draw=none, chainingStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_100/chaining_table.txt};

    \addplot[draw=none, warpcoreStyleFill, x=op, y=probes]   table {data/results/sawtooth_probe_100/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

  \end{axis}
  \end{tikzpicture}
  \caption{Performance for expansions only}
  \label{fig::probe_100}
\end{subfigure}

==> figures/lf_probe/lf_probe_figures.tex <==
\begin{figure*}[hbt!]
    %\ref{lfProbeLegend}
    \centering
    \input{figures/lf_probe/lf_probe_insertion}\hfill
    \input{figures/lf_probe/lf_probe_query}\hfill
    \input{figures/lf_probe/lf_probe_remove}

    \caption{Load factor probe results. The x-axis the the load factor of the hash table, with each table initialized to hold 100 million keys, and the y-axis is the average number of cache line touches. The left graph is probe counts for insertion, the middle graph represents queries, and the right graph is deletions.}
    \label{fig::lf_probe_all}
\end{figure*}

==> figures/lf_probe/lf_probe_insertion.tex <==
\begin{subfigure}{.3\textwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    LFProbePlot,
    %ymode = log,
    %symbolic x coords={Insertion,Upsert,Query, Deletion},
    enlarge x limits=0.15,
    legend to name=lfProbeLegend,
    legend columns = 2,
    xlabel={Load factor}
    ]

    %BETA OuroborosPVA OuroborosCS
    \addplot[p2ExtStyle, x=lf, y=insert]   table {data/results/lf_probe/p2_hashing_external.txt};

    % \addplot[p2IntStyle, x=lf, y=insert]   table {data/results/lf_probe/p2_hashing_internal.txt};

    \addplot[cuckooStyle, x=lf, y=insert]   table {data/results/lf_probe/cuckoo_hashing.txt};


    \addplot[doubleStyle, x=lf, y=insert]   table {data/results/lf_probe/double_hashing.txt};

    \addplot[ihtStyle, x=lf, y=insert]   table {data/results/lf_probe/iht_p2_hashing.txt};

    \addplot[ihtMetaStyle, x=lf, y=insert]   table {data/results/lf_probe/iht_p2_metadata_full_hashing.txt};

    \addplot[chainingStyle, x=lf, y=insert]   table {data/results/lf_probe/chaining_table.txt};

    %\addplot[warpcoreStyle, x=lf, y=insert]   table {data/results/lf_probe/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

    \addplot[p2MetaStyle, x=lf, y=insert] table {data/results/lf_probe/p2_hashing_metadata.txt};

    % \addplot[cuckooStyle, x=lf, y=insert]   table {data/results/lf_probe/cuckoo_hashing.txt};

    \legend{P2 Hashing (External), P2 Hashing (Internal), Double Hashing, Iceberg Hashing, Chaining, P2 Metadata}
  \end{axis}
  \end{tikzpicture}
  \caption{Insertion}
  \label{fig:lf_insert_probe}
\end{subfigure}

==> figures/lf_probe/lf_probe_query.tex <==
\begin{subfigure}{.3\textwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    LFProbePlot,
    %ymode = log,
    %symbolic x coords={Insertion,Upsert,Query, Deletion},
    table/col sep = comma,
    enlarge x limits=0.15,
    xlabel={Load factor}
    ]

    %\addplot[p2ExtStyle, x=lf, y=query]   table {data/results/lf/p2_hashing_external.txt};

    %\addplot[p2ExtStyle, x index=0, y index=2] table {data/results/lf/p2_hashing_external.txt};
    \addplot[p2ExtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/p2_hashing_external.txt};

    % \addplot[p2IntStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/p2_hashing_internal.txt};
    
    \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/cuckoo_hashing.txt};


    \addplot[doubleStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/double_hashing.txt};

    \addplot[ihtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/iht_p2_hashing.txt};

    \addplot[ihtMetaStyle]  table[x expr=\thisrowno{0}, y expr=\thisrowno{2}]{data/results/lf_probe/iht_p2_metadata_full_hashing.txt};

    \addplot[chainingStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/chaining_table.txt};

    %\addplot[warpcoreStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

    \addplot[p2MetaStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/p2_hashing_metadata.txt};


    % \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/cuckoo_hashing.txt};




  \end{axis}
  \end{tikzpicture}
  \caption{Query}
  \label{fig:lf_probe_query}
\end{subfigure}

==> figures/lf_probe/lf_probe_remove.tex <==
\begin{subfigure}{.3\textwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    LFProbePlot,
    %ymode = log,
    %symbolic x coords={Insertion,Upsert,Query, Deletion},
    table/col sep = comma,
    enlarge x limits=0.15,
    xlabel={Load factor}
    ]

    %\addplot[p2ExtStyle, x=lf, y=query]   table {data/results/lf/p2_hashing_external.txt};

    %\addplot[p2ExtStyle, x index=0, y index=2] table {data/results/lf/p2_hashing_external.txt};
    \addplot[p2ExtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{3}] {data/results/lf_probe/p2_hashing_external.txt};

    % \addplot[p2IntStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{3}] {data/results/lf_probe/p2_hashing_internal.txt};
    
    \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{3}] {data/results/lf_probe/cuckoo_hashing.txt};


    \addplot[doubleStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{3}] {data/results/lf_probe/double_hashing.txt};

    \addplot[ihtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{3}] {data/results/lf_probe/iht_p2_hashing.txt};

    \addplot[ihtMetaStyle]  table[x expr=\thisrowno{0}, y expr=\thisrowno{3}]{data/results/lf_probe/iht_p2_metadata_full_hashing.txt};
        
    \addplot[chainingStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{3}] {data/results/lf_probe/chaining_table.txt};

    %\addplot[warpcoreStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

    \addplot[p2MetaStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{3}] {data/results/lf_probe/p2_hashing_metadata.txt};


    % \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/lf_probe/cuckoo_hashing.txt};




  \end{axis}
  \end{tikzpicture}
  \caption{Deletion}
  \label{fig:lf_probe_remove}
\end{subfigure}

==> figures/scaling/scaling_bght_combined.tex <==
\begin{figure*}[t]
    \centering
    \input{figures/scaling/scaling_query}%
    \input{figures/scaling/scaling_probe}%
    \input{figures/bght_comp/bght_query}%
    \input{figures/bght_comp/bght_probe}

    

    \caption{Query and probe performance when scaling the tables.}
    \label{fig::scaling_bght_mixed}
\end{figure*}

==> figures/scaling/scaling_probe.tex <==
\begin{subfigure}{.4\textwidth}

\begin{tikzpicture}
  \centering
  \begin{axis}[
    scalingProbePlot,
    %ymode = log,
    %symbolic x coords={Insertion,Upsert,Query, Deletion},
    xmode=log,
    log basis x={10},
    table/col sep = comma,
    enlarge x limits=0.15,
    xlabel={\# Items Inserted}
    ]

    %\addplot[p2ExtStyle, x=scaling, y=query]   table {data/results/scaling/p2_hashing_external.txt};

    %\addplot[p2ExtStyle, x index=0, y index=2] table {data/results/scaling/p2_hashing_external.txt};
    \addplot[p2ExtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/scaling_probe/p2_hashing_external.txt};

    % \addplot[p2IntStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/scaling_probe/p2_hashing_internal.txt};
    
    \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/scaling_probe/cuckoo_hashing.txt};


    \addplot[doubleStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/scaling_probe/double_hashing.txt};

    \addplot[ihtStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/scaling_probe/iht_p2_hashing.txt};

    \addplot[ihtMetaStyle]  table[x expr=\thisrowno{0}, y expr=\thisrowno{2}]{data/results/scaling_probe/iht_p2_metadata_full_hashing.txt};

    \addplot[chainingStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/scaling_probe/chaining_table.txt};

    %\addplot[warpcoreStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/scaling_probe/warpcore_hashing.txt};
    %\addplot[draw=none, fill=green!30, x=op, y=perf]   table {data/orkut_CUDA.txt};

    \addplot[p2MetaStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/scaling_probe/p2_hashing_metadata.txt};



    % \addplot[cuckooStyle] table[x expr=\thisrowno{0}, y expr=\thisrowno{2}] {data/results/scaling_probe/cuckoo_hashing.txt};




  \end{axis}
  \end{tikzpicture}
  \caption{Scaling Probe}
  \label{fig:scaling_probe}
\end{subfigure}

==> figures/tables/adversarial.tex <==
%\definecolor{cellgreen}{rgb}{0.1,0.1,0.1}

\begin{table}[t]
    \begin{center}
    \begin{tabular}{c|c}
    \toprule
    Hash Table & Passes Adversarial Test\\
    \midrule
    Slabhash & \cellcolor{red!25}No \\
    \double & \cellcolor{green!25}Yes \\
    \doubleMeta & \cellcolor{green!25}Yes \\
    \iceberg & \cellcolor{green!25}Yes \\
    \icebergMeta & \cellcolor{green!25}Yes \\
    \power & \cellcolor{green!25}Yes \\
    \meta & \cellcolor{green!25}Yes \\
    \cuckoo & \cellcolor{green!25}Yes \\
    \chaining & \cellcolor{green!25}Yes \\
    \bottomrule
    \end{tabular}
\end{center}
\caption{Adversarial benchmark results. Tables are initialized to have 1,000,000 buckets. Tables only pass the test if no buckets show a race condition. 
}
\label{tab:adversarial}
\end{table}

==> figures/tables/concurrency.tex <==
% \begin{table}
%     \begin{center}
%     \begin{tabular}{|c| c c|}
%     \toprule
%     Hash Table & Concurrent (MOps/S) & Phased (MOps/S)\\
%     \midrule
%     \double & 2062.89 & 3233.83 \\
%     \iceberg & 1392.85 & 1406.06 \\

%     \icebergMeta & 2398.93 & 2906.61 \\
%     \chaining &  1775.82 & 2268.16 \\
%     \cuckoo & 2696.99 & 3362.39 \\
%     \power & 1451.642 & 1472.27 \\
%     \meta & 2605.54 & 2929.58 \\
%     \doubleMeta & 2887.18 & 2922.50 \\
%     BCHT (BGHT) & ? &  1707.79 \\
%     P2BHT (BGHT) & ? & 2546.68
%     \bottomrule
%     \end{tabular}
% \end{center}

% \label{tab:space_usage}
% \end{table}



\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{ c | c | c | c }
    \toprule
    \bf Hash Table & Concurrent & Phased & overhead \\
     & (MOps/S) & (MOps/S) & \% \\
    \midrule
    \double & 2062.89 & 3233.83 & 56.7\\
    \doubleMeta & 2887.18 & 2922.50 & 1.22\\
    \iceberg & 1392.85 & 1406.06 & 0.95\\
    \icebergMeta & 2398.93 & 2906.61 & 21.2\\
    \power & 1451.642 & 1472.27 & 1.42 \\
    \meta & 2605.54 & 2929.58 & 12.43\\
    \cuckoo & 2696.99 & 3362.39 & 24.67\\
    \chaining &  1775.82 & 2268.16 & 27.72\\
    BCHT (BGHT) & - &  1707.79 & - \\
    P2BHT (BGHT) & - & 2546.68 & -\\
    \bottomrule
    \end{tabular}
    }
    \caption{Average cost of concurrent vs phased implementation. Results are presented as the average performance when loading to 90\% and in MOps/second. The phased approach is identical to the concurrent implementation, but with locks removed and all load instructions made cacheable. BCHT and P2BHT are the bucketed cuckoo hash table and Power-of-two-choices hash table from BGHT~\cite{BGHT}.}
    \label{tab:concurrency}
    \vspace{-1.5em}
\end{table}


==> figures/tables/flow_table.tex <==

%counters
\def\basiceval#1{\the\numexpr#1\relax}

\begin{figure*}[ht]

\begin{tikzpicture}[scale=.8]


    % \node[minimum size=8mm] at (9.5,2) {\large Configuration Tested (Bucket Size-Tile Size)};

  %\node[minimum size=6mm] at (10, 0){16\_2}
  \foreach \a [count=\i] in {4-1,4-2,4-4,8-1,8-2,8-4,8-8,16-1,16-2,16-4,16-8,16-16, 32-1, 32-2, 32-4, 32-8, 32-16, 32-32} {
    \node[minimum size=8mm] at (\i,0) {\a};
  }

  \foreach \y [count=\n] in {
      {0,0,0,0,0,0,0,0,0,0,0,0,381,540,938,1153,1075,838},
      %{0,0,0,1478,0,0,0,143,1597,0,0,0,1250,1338,1750,0,0,0},
      {857,1285,2199,583,905,1661,2226,309,525,984,1384,1545,164,281,547,763,879,911},
      %{0,0,0,1338,0,0,0,1423,1589,0,0,0,1132,1245,1738,0,0,0},
      {0,0,0,0,0,0,0,650,862,1418,1663,1462,369,509,891,1106,1047, 831},
      %{0,0,0,1450,0,0,0,1415,1600,0,0,0,1241,1327,1741,0,0,0},
      {1236,1606,1734,869,1149,1580,1690,566,777,1179,1472,1221,335,487,810,1041,1004,766},
      {1316,1692,2339,1074,1270,1883,1834,772,854,1361,1474,1158,428,523,891,1051,922,677},
    } {
      % column labels
      % \ifnum\n<10
      %   \node[minimum size=6mm] at (\n, 0) {\n};
      % \fi
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \def\k{22};
        \def\e{\basiceval{\x/\k}};
        \node[fill=yellow!\e!purple, minimum size=8mm, text=white] at (\m,-\n) {\x};
      }
    }

  % row labels
  \foreach \a [count=\i] in {\power,\double,\iceberg,\chaining,\cuckoo} {
    \node[minimum size=8mm] at (-1,-\i) {\a};
  }
\end{tikzpicture}

\label{heatmap}
\caption{Heatmap of hash table performance as a measure of bucket and tile
  size. Each row is a hash table and the each column is a possible combination
  of bucket and tile size, starting with buckets of 4 key-value pairs and one
  thread per tile (4-1) and ending with buckets of 32 key-value pairs and 32
threads per tile (32-32). The numerical result presented is the average
workload throughput comprising of insertions, deletions, and queries in
millions of operations per second. \prashant{We can remove this figure and discuss the numbers in text.}}
  
\end{figure*}



%old version


%counters
% \def\basiceval#1{\the\numexpr#1\relax}

% \begin{figure*}[t]

% \begin{tikzpicture}[scale=.8]


%     \node[minimum size=8mm] at (9.5,2) {\large Configuration Tested (Bucket Size-Tile Size)};

%   %\node[minimum size=6mm] at (10, 0){16\_2}
%   \foreach \a [count=\i] in {4-1,4-2,4-4,8-1,8-2,8-4,8-8,16-1,16-2,16-4,16-8,16-16, 32-1, 32-2, 32-4, 32-8, 32-16, 32-32} {
%     \node[minimum size=8mm] at (\i,0) {\a};
%   }

%   \foreach \y [count=\n] in {
%       {1449,1929,2638,1078,1411,2135,2340,685,913,1478,1723,1485,381,540,938,1153,1075,838},
%       %{0,0,0,1478,0,0,0,143,1597,0,0,0,1250,1338,1750,0,0,0},
%       {857,1285,2199,583,905,1661,2226,309,525,984,1384,1545,164,281,547,763,879,911},
%       %{0,0,0,1338,0,0,0,1423,1589,0,0,0,1132,1245,1738,0,0,0},
%       {1382,1843,2622,1029,1344,2067,2283,650,862,1418,1663,1462,369,509,891,1106,1047, 831},
%       %{0,0,0,1450,0,0,0,1415,1600,0,0,0,1241,1327,1741,0,0,0},
%       {1236,1606,1734,869,1149,1580,1690,566,777,1179,1472,1221,335,487,810,1041,1004,766},
%       {1316,1692,2339,1074,1270,1883,1834,772,854,1361,1474,1158,428,523,891,1051,922,677},
%     } {
%       % column labels
%       % \ifnum\n<10
%       %   \node[minimum size=6mm] at (\n, 0) {\n};
%       % \fi
%       % heatmap tiles
%       \foreach \x [count=\m] in \y {
%         \def\k{25};
%         \def\e{\basiceval{\x/\k}};
%         \node[fill=yellow!\e!purple, minimum size=8mm, text=white] at (\m,-\n) {\x};
%       }
%     }

%   % row labels
%   \foreach \a [count=\i] in {\power,\double,\iceberg,\chaining,\cuckoo} {
%     \node[minimum size=8mm] at (-1,-\i) {\a};
%   }
% \end{tikzpicture}

% \label{heatmap}
% \caption{Heatmap of performance as a measure of bucket and tile size. The Y-axis is table designs, and the X-axis is every possible combination of bucket and tile size, with each value being in the form $A-B$ where $A$ is the bucket size and $B$ is the tile size. Results presented are the average performance between insertions, deletions, and queries in megaops per second.}
  
% \end{figure*}


==> figures/tables/space.tex <==
\begin{table}[t]
    \begin{center}
    \begin{tabular}{c|c|c}
    \toprule
    Hash Table & Space Usage (GB) & Space Efficiency (\%)\\
    \midrule
    \double & 1.601 & 89.91\%\\
    \doubleMeta & 1.800 & 79.98\% \\
    \iceberg & 1.600 & 89.98\% \\
    \icebergMeta & 1.800 & 79.99\% \\
    \power & 1.600 & 89.98\% \\
    \meta & 1.800 & 79.98\% \\
    \cuckoo & 1.601 & 89.91\% \\
    \chaining &  3.441 & 41.84\% \\
    \bottomrule
    \end{tabular}
\end{center}
\caption{Total space usage for various hash tables. 
% The space usage is calculated at the end of the aging benchmark (1000 iterations). 
Each hash table is initialized to 100M slots for 16 byte key-value pairs, and space is measured after inserting 90M keys. Space efficiency is a measure of the total space usage of the table compared to the minimum required to store the keys.
}
\label{tab:space_usage}
\end{table}

==> figures/tables/sptc.tex <==

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{| c | c c |}
    \toprule
    \bf Table & Table Construction (sec) & Contraction (sec)\\
    \midrule
    \double & .029 & 2.49 \\
    \doubleMeta & .032 & 3.08 \\
    \chaining & .014 & 3.55 \\
    \iceberg & .026 & 4.05 \\
    \icebergMeta & .027 & 3.65 \\
    \power & .026 & 4.63 \\
    \meta & .026 & 3.58 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Sparse contraction of the NIPS tensor with itself. Table construction is the duration of time in seconds required to convert the COO Y matrix into a hash table. Contraction is the duration in seconds required to contract the tensors and accumulate the result. \prashant{cuckoo missing.}}
    \label{tab:sptc}
    \vspace{-1.5em}
\end{table}


==> prev.tex <==
\section{A brief history of GPU hash tables}

%\section{Previous work}
% GPU tables to discuss
% \begin{itemize}
%     \item \cite{gpuHashingVoxels} 2014 Describes a simple way to construct gpu hash tables for voxel storage. Graphics application that only wants to store live voxels for dynamic spacial data
%     \item \cite{gpuHashingThesis}: 2011 Thesis from one of John Owen's students, covers most of the basic hash table designs: open addressing, chaining, cuckoo, cuckoo with stashes.
%     \item \cite{stadiumHashing} utilizes an \textit{ticketing board} system on top of double hashing to claim locations and queries. 1+ bits are given to each item in stadium hashing to resolve collisions early, with one bit always reserved in a ticket to mark it as available. Improved over old papers \^ by allowing concurrent insertions and queries as the table is stable.
% \end{itemize}

The first paper to focus on hash table design and performance on the GPU was Alcantara et al.~\cite{realTimeHashingGPU} published in 2009. This paper presents a bulk-synchronous algorithm for hash table construction that separates keys into large buckets of 512 items and uses cuckoo hashing to resolve collisions inside of the buckets. This work was further improved in Alcantara~\cite{gpuHashingThesis} which included designs for linear probing, quadratic probing, chaining, and a cuckoo hash table with stashing. Khorasani et Al.~\cite{stadiumHashing} then proposed stadium hashing, a bulk-synchronous table based on double hashing that allowed for insertions and queries to occur simultaneously.

The first table to edge out of the bulk-synchronous framework was warpcore from Jünger et al.~\cite{warpcore} which used a tiling strategy to efficiently partition warps for operations.

The current state of the art have all been released after warpcore. In this section, we separate the state of the art into bulk-synchronous, static, and concurrent hash tables.

\subsection{Bulk-Synchronous Hash Tables}

\para{SlabHash} SlabHash~\cite{slabhash} is a concurrent, dynamic hash table based on chaining. The table uses atomicCAS to emplace keys into buckets, and maintains a custom allocation scheme called slabAllocator to request new bucket allocations efficiently. Slabhash uses the atomicCAS instruction to atomically emplace and delete items from the table. It does not use locking of any kind when inserting items. In \cref{subsec:adverserial} we discuss this design in more detail and highlight the necessity of locking in dynamic hash table designs.

\para{Warpcore} Warpcore~\cite{warpcore} and its previous implementation warpdrive~\cite{warpdrive} are bulk-synchronous double hashing hash tables. These tables have a warp-level implementation and were the first GPU hash table designs to utilize cooperative groups for tiling. Atomics are used to prevent insertion into the same slot, but these tables are explicitly not dynamic: the table offers no guarantee of unique insertion of keys and they explicitly do not support different operations occurring within the same kernel.


\para{DyCuckoo} DyCuckoo~\cite{dyCuckoo} is a bulk-synchronous hash table that only performs batched operations. The design of the table is based on 2-way bucketed cuckoo hashing. In this design, called \textit{2-in-d} hashing, the full hash table is composed of \textit{d} different subtables. Keys hash to exactly one location inside of a subtable, and instead of cuckooing between buckets, keys cuckoo between different subtables. This design allows the table resized incrementally, as a subtable can be resized without requiring a rehash of the keys in other subtables. The API for this table is entirely host-controlled.


\subsection{Static Hash Tables}

\para{Better GPU Hash Tables} Better GPU Hash Tables (BGHT)~\cite{BGHT} presents several hash tables designs optimized for use on a GPU. These tables are all \textbf{static}, meaning that keys are inserted during construction of the table and are never modified. This paper finds that the \textbf{probe count}, the number of cache lines touched during an operation, is the main factor that influences hash table performance, with tables that have smaller probe counts outperforming those with larger probe counts. They further find that the best hash table design for GPUs is a bucketed cuckoo hash table as it requires an average of 1.43 probes per query even at 90\% load factor.

\subsection{Concurrent hash tables}
\para{GELHash} Up to this point, the only fully concurrent hash table for GPUs in the literature is GELHash. GELHash~\cite{GelHash} is a chaining hash table that utilizes reader-writer locks adapted from~\cite{GPULocking} to be fully concurrent. Like SlabHash~\cite{slabhash}, GELHash uses chaining inside of buckets, with each bucket being represented by a bucketized linked list. The table offers two different operation styles, with operations occurring at either the thread level or the warp level. This is equivalent to using tile sizes of 1 or 32. A public implementation of this table is not available.
